Improved Approximations for Ultrametric Violation Distance

We study the Ultrametric Violation Distance problem introduced by Cohen-Addad, Fan, Lee, and Mesmay [FOCS, 2022]. Given pairwise distances $x\in \mathbb{R}_{>0}^{\binom{[n]}{2}}$ as input, the goal is to modify the minimum number of distances so as to make it a valid ultrametric. In other words, this is the problem of fitting an ultrametric to given data, where the quality of the fit is measured by the $\ell_0$ norm of the error; variants of the problem for the $\ell_\infty$ and $\ell_1$ norms are well-studied in the literature. Our main result is a 5-approximation algorithm for Ultrametric Violation Distance, improving the previous best large constant factor ($\geq 1000$) approximation algorithm. We give an $O(\min\{L,\log n\})$-approximation for weighted Ultrametric Violation Distance where the weights satisfy triangle inequality and $L$ is the number of distinct values in the input. We also give a $16$-approximation for the problem on $k$-partite graphs, where the input is specified on pairs of vertices that form a complete $k$-partite graph. All our results use a unified algorithmic framework with small modifications for the three cases.

==> app-related.tex <==
\label{sec:related}

\paragraph{Fitting ultrametrics with other objectives.}
The problem of fitting ultrametrics for $\ell_{\infty}$ and $\ell_1$ norms are well-studied in the literature.
Farach et al.~\cite{farach1993robust} gives a polynomial-time algorithm that solves exactly for the $\ell_{\infty}$ objective.
However, for the $\ell_p$ objective ($1\leq p<\infty$), the APX-hardness of the problem can be derived from the APX-hardness of \CClust~\cite{DBLP:journals/jcss/CharikarGW05}.
There is a line of works studying its approximation algorithms~\cite{harb2005approximating,DBLP:journals/siamcomp/AilonC11,DBLP:conf/focs/Cohen-Addad0KPT21}.
The state-of-the-art algorithms are an $O(1)$-approximation algorithm for $\ell_1$ norm and $O((\log n\log \log n)^{1/p})$-approximations for $\ell_p$ norms ($1< p<\infty$).
A lot of other objectives and assumptions are also considered in the literature of fitting ultrametrics, including the maximization version~\cite{duggal2013resolving,DBLP:conf/focs/Cohen-AddadFLM22}, the outlier deletion version~\cite{sidiropoulos2017metric}, multiplicative distortion version~\cite{di2015finding} and assuming the input is on high-dimensional Euclidean space~\cite{cohen2020efficient,cohen2021improving}.

\paragraph{Fitting metrics and tree metrics.} 
% There is also a line of literature on fitting a metric or tree metric to given data. 
Brickell et al.~\cite{brickell2008metric} formulated the problem of fitting metrics to a given data with $\ell_p$ objective for $1\leq p\leq \infty$, which can be solved exactly in polynomial-time via linear or convex programs.
The $\ell_0$ version was recently introduced and studied~\cite{gilbert2017if,fan2018metric,fan2020generalized,DBLP:conf/focs/Cohen-AddadFLM22}, culminating in an $O(\log n)$-approximation algorithm that runs in $O(n^3)$ time.

% The literature studying fitting tree metrics is much richer. 
On the other hand, Cavalli-Sforza and Edwards~\cite{cavalli1967phylogenetic} introduced the tree fitting problem.
If there is a tree metric exactly fitting the data, the structure can be found in polynomial time~\cite{waterman1977additive}.
However, if there is no such tree metric, the problem for any $\ell_p$ objective ($1\leq p \leq \infty$) is APX-hard~\cite{agarwala1998approximability,DBLP:journals/jcss/CharikarGW05}.
In addition, Agarwala et al.~\cite{agarwala1998approximability} give a general reduction from tree metrics to ultrametrics, only losing a factor of $3$.
The state-of-art algorithms are then a 3-approximation for $\ell_{\infty}$ norm, an $O(1)$-approximation algorithm for $\ell_1$ norm and $O((\log n\log \log n)^{1/p})$-approximations for $\ell_p$ norms ($1< p<\infty$).
However, we are not aware of any work considering fitting tree metrics for the $\ell_0$ norm.
% Other related works involve fitting line metrics~\cite{},  

\paragraph{Correlation clustering.} 
As mentioned before, \CClust has been extensively studied.
Bansal, Blum and Chawla~\cite{bansal2004correlation} introduced the problem and gave a constant factor approximation.
Later, it was improved by~\cite{DBLP:journals/jcss/CharikarGW05,DBLP:journals/jacm/AilonCN08,DBLP:conf/stoc/ChawlaMSY15,DBLP:conf/focs/Cohen-AddadLN22}.
The current best algorithm is a $(1.994+\eps)$-approximation based on the Sherali-Adams hierarchy.
And, this problem is APX-hard~\cite{DBLP:journals/jcss/CharikarGW05}.
A number of variants of \CClust have also been studied. 
Among those, works regarding the weighted cases include the general version~\cite{demaine2006correlation,DBLP:journals/jcss/CharikarGW05}, the version with probability constraints~\cite{gionis2007clustering,DBLP:journals/jacm/AilonCN08,DBLP:conf/stoc/ChawlaMSY15} and the version for asymmetric error costs~\cite{jafarov2020correlation}.

==> future.tex <==
\begin{enumerate}
    \item Consider rounding the Sherali-Adams
    \item 
\end{enumerate}

==> obsolete.tex <==
% \begin{theorem}
% \label{thm:9-approx}
%     With parameter $\alpha=\frac23$, Algorithm~\ref{alg:pivot} is a 9-approximation algorithm for ultrametric violation distance. 
% \end{theorem}



\begin{lemma}
    \label{lem:M-bound-by-B}
    With the below definitions of $B_{i,j,t}$, for any triangle $t\in \binom{[n]}{3}$ and any type $\theta\in [5]$, 
    $$\sum_{(i,j)\in t} \expect[M_{i,j,t}|\mathcal{A}_t^{\theta}]\leq 2\sum_{(i,j)\in t} c^*(i,j)\cdot \expect[B_{i,j,t}|\mathcal{A}_t^{\theta}]~.$$
\end{lemma}

Taking expectations on both sides and summing over all possible $i,j,t$, we have
\begin{align*}
    \sum_{t\in \binom{[n]}{3}}\sum_{(i,j)\in t} \expect[M_{i,j,t}] \leq 2\sum_{(i,j)\in \binom{[n]}{2}} \bigg(\sum_{t:(i,j)\in t} \expect[B_{i,j,t}]\bigg)\cdot c^*(i,j)~.
\end{align*}
And we have the following corollary about the approximation ratio of the algorithm.
\begin{corollary}
\label{cor:2beta+3-approx}
    Suppose $\beta>0$ satisfies $\beta\geq \sum_{t:(i,j)\in t} \expect[B_{i,j,t}]$ for any instance and for any $(i,j)\in \binom{[n]}{2}$. Then, Algorithm~\ref{alg:pivot} is an expected $(2\beta+3)$-approximation algorithm for ultrametric violation distance.
\end{corollary}



\begin{lemma}
    \label{lem:improved-M-bound-by-B}
    With the below definitions of $B_{i,j,t}$, for any triangle $t\in \binom{[n]}{3}$, 
    \begin{align}
        \label{eqn:improved-M-bound-by-B}
        \sum_{(i,j)\in t} \expect[M_{i,j,t}|\mathcal{A}_t]\leq \sum_{(i,j)\in t} c^*(i,j)\cdot \expect[B_{i,j,t}|\mathcal{A}_t]~.
    \end{align}
\end{lemma}

\begin{lemma}
    \label{lem:improved-bound-of-B}
    With the below definition of $B_{i,j,t}$, for any $b>0$, conditioning on $B_{i,j,t}=b$ in a recursive call, the probability that $i$ and $j$ will appear in different clusters is lower bounded by $f_{i,j}\cdot b$, where 
    \begin{align*}
        f_{i,j} 
        =
        \begin{cases}
           \min\{\frac{\alpha}{3},\frac{1-\alpha}{2}\}  & \text{$(i,j)$ is $\lowerr$}\\
           \frac{\alpha}{2}  & \text{$(i,j)$ is $\highrand$}\\
           1-\alpha  & \text{$(i,j)$ is $\highdet$}
        \end{cases}
    \end{align*}
\end{lemma}


Suppose $y$ is the LP solution inside the recursive call in which $\mathcal{A}_t$ happens. According to $y$, we can classify $\mathcal{A}_t$ into five types by the number of deterministic edges on $t$ and their deterministic weights, and let $\mathcal{A}_t^{\theta}$ be the event when $\mathcal{A}_t$ is classified into the $\theta$-th type. In addition, we define some of the backward edges as dangerous in $\mathcal{A}_t$, where the definition varies with the type of $\mathcal{A}_t$. Let $B_{i,j,t}$ be the event that $(u,v)$ is a dangerous backward edge in $\mathcal{A}_t$. We will introduce the definition of the types and the cases we define the backward edge as dangerous later. With these definitions, we can bound the expected values of $M_{i,j,t}$s according to the expected values of $B_{i,j,t}$s. 

Suppose $y$ is the LP solution inside the recursive call in which $\mathcal{A}_t$ happens. 
According to $y$, we can classify $\mathcal{A}_t$ into five types by the number of deterministic edges on $t$ and their deterministic weights, and we shall charge the backward edge $(u,v)$ of $\mathcal{A}_t$ by $B_{u,v,t}c^*(u,v)$, where the weight $B_{u,v,t}$ varies with the type of $\mathcal{A}_t$. We will introduce our specific definitions of the types and $B_{u,v,t}$s later in this section. The goal of our definition is to upper bound the expected values of $M_{i,j,t}$s according to the expected values of $B_{i,j,t}$s (Lemma~\ref{lem:improved-M-bound-by-B}), and at the same time ensure some property (Lemma~\ref{lem:improved-bound-of-B}) so that we can upper bound for the expected sum of $B_{i,j,t}$s (Corollary~\ref{lem:bound-of-sum-B}). 

\subsection{Bounding the Expected Number of Dangerous Appearances}

To upper bound the expected number of dangerous appearances, a key observation is that when an edge appears dangerously in a recursive call, if the other two edges are both deterministic, their weights should be unequal. The observation can be verified by the definitions of $B_{i,j,t}$s in the last subsection. As a result of this observation, we can derive the following lemma:
\begin{lemma}
    \label{lem:prob-disappear-after-appear}
    Fix an edge $(i,j)$ and another vertex $k\neq i,j$. Let $t=\{i,j,k\}$ be the triangle including all these three vertices. In any recursive call where $k$ is chosen as the pivot, conditioned on $B_{i,j,t}=1$, the probability that vertex $i,j$ appears in the same following recursive call is at most $\frac23$. Or equivalently, in the recursive call, the probability that there exists an $\ell\in [L]$ such that $i,j\in V_{\ell}$ is at most $\frac23$.
\end{lemma}
\begin{proof}
We will show the lemma by discussing the types of $(i,k)$ and $(j,k)$. Suppose the LP solution in the recursive call is $y$.

\paragraph{Both are deterministic.} According to the observation, the deterministic edges have different weights. Therefore, $i$ and $j$ will appear in different $V_{\ell}$s and the probability considered in the lemma is $0$.

\paragraph{Exactly one of them is deterministic.} W.l.o.g, suppose $(i,k)$ is deterministic and its weight level in the recursive call is $\ell$. $i$ appears in $V_{\ell}$ in the recursive call. According to the algorithm, with probability $\Delta y_{\ell}(j,k)$, the random edge weight of $(j,k)$ equals $w_\ell$ and $j$ also appears in $V_{\ell}$. Since edge $(j,k)$ is random, according to the definition of random edges, $\Delta y_{\ell}(j,k)\leq \frac23$. Therefore, the probability considered in the lemma is at most $\frac23$. 

\paragraph{Both are random.} $i$ and $j$ appear in the same $V_\ell$ only when the random weights of edges $(i,k)$ and $(j,k)$ are the same. According to the algorithm, the probability that $x'(i,k)=x'(j,k)$ is
\begin{align*}
    \sum_{\ell\in [L]} \Delta y_\ell(i,k)\Delta y_\ell(j,k) \leq \sum_{\ell\in [L]} \frac{2}3 \Delta y_{\ell}(j,k) = \frac23~.
\end{align*}
Therefore, the probability considered in the lemma is at most $\frac23$.
\end{proof}

Next, we prove the expected number of dangerous appearances of any edge $(i,j)$ is upper bounded by $3$ in any recursive call (and its subsequent calls) with any instance $n,L,x,w,y$ by induction on $n$. The base case is when $n\leq 2$, and the induction hypothesis holds because the algorithm simply returns the input $x$. Suppose the induction hypothesis holds for any instance with $n\leq n_0$. Consider any instance with $n=n_0+1$. Suppose the random pivot chosen in the recursive call is $k$ and let $t=\{i,j,k\}$. For each edge $(i,j)\in \binom{[n_0+1]}{2}$, we discuss the following cases:
\begin{enumerate}
    \item If $B_{i,j,t}=1$, according to Lemma~\ref{lem:prob-disappear-after-appear}, with probability at most $\frac23$, $i,j$ will appear in the same $V_{\ell}$. Otherwise, $i,j$ will appear in different recursive calls, and edge $(i,j)$ will no longer appear as dangerous in any subsequent calls. If $i,j$ appears in the same $V_{\ell}$, because $V_\ell\subseteq [n_0+1]\setminus \{k\}$, they will appear in one subsequent (possibly random) recursive call with $n\leq n_0$. By the induction hypothesis, the expected number of dangerous appearances of $(i,j)$ in any of the possible subsequent calls is upper bounded by $3$. In total, the expected number of dangerous appearances of $(i,j)$ in this call is upper bounded by $1+\frac{2}{3}\cdot 3 + \frac13\cdot 0=3$.
    \item If $B_{i,j,t}=0$, $(i,j)$ will only appear as dangerous in subsequent recursive calls with $n\leq n_0$, and by the induction hypothesis, the expected number of dangerous appearances of $(i,j)$ in this call is upper bounded by $3$.
\end{enumerate}
Taking expectations on $k$, we can prove that $(i,j)$ does not appear as dangerous for more than $3$ times in expectation. Combining with Corollary~\ref{cor:2beta+3-approx}, we finish the proof of Theorem~\ref{thm:9-approx}.

% For any recursive call with input $n$ and other input $\mathcal{I}=\{L,x,w,y\}$, let $B_{i,j}(n,\mathcal{I})$ be the number of dangerous appearance of $(i,j)$ in the recursive and the following recursive call, and let $\mathcal{B}_{i,j}(n,\mathcal{I})$ be the event that $(i,j)$ appears dangerously in the triangle including $i,j$ and the pivot vertex of the recursive call. According to the algorithm and Lemma~\ref{lem:prob-disappear-after-appear}, 
% \begin{align*}
%     \expect[B_{i,j}(n,\mathcal{I})] 
%     \leq 
%     &
%     \Pr[\mathcal{B}_{i,j}(n,\mathcal{I})] 
%     \cdot 
%     \bigg(1+\frac{2}3\cdot \expect_{n',\mathcal{I}'\sim ALG}\big[B_{i,j}(n',\mathcal{I'})
%     \,\big|\,
%     \mathcal{B}_{i,j}(n,\mathcal{I})\big]\bigg) 
%     \\
%     &
%     +
%     \big(1-\Pr[\mathcal{B}_{i,j}(n,\mathcal{I})]\big)
%     \cdot 
%     \expect_{n',\mathcal{I}'\sim ALG}\big[B_{i,j}(n',\mathcal{I'})
%     \,\big|\,
%     \neg \mathcal{B}_{i,j}(n,\mathcal{I})\big] 
% \end{align*}
% where $n',$


\paragraph{Three Deterministic Edges (Type 1).}
In this type, $\Delta y_{\ell^*(i,j)}(i,j), \Delta y_{\ell^*(i,k)}(i,k), \Delta y_{\ell^*(j,k)}(j,k)> \frac23$. We can prove $M_{i,j,t}=M_{i,k,t}=M_{j,k,t}=0$ by showing that $w_{\ell^*(y,i,j)}, w_{\ell^*(y,i,k)}, w_{\ell^*(y,j,k)}$ satisfies the ultrametric inequality. Note that the violation of the ultrametric inequality happens only when two weights are strictly less than the other one. Since the edges are deterministic, we have
\begin{align*}
\forall u\neq v\in t, %\{i,j,k\}, 
\quad
y_{\ell^*(u,v)-1}(u,v) < \frac13, 
\;
y_{\ell^*(u,v)}(u,v) > \frac23~.
\end{align*}
If there is a violation of the ultrametric inequality, w.l.o.g. say $\ell^*(y,j,k)<\ell^*(y,i,j),\ell^*(y,i,k)$, we can find a violation of the triangle inequality in $y$ on level $\ell^*(j,k)$:
\begin{align*}
y_{\ell^*(j,k)}(i,j)+y_{\ell^*(j,k)}(i,k) 
\leq 
y_{\ell^*(i,j)-1}(i,j)+y_{\ell^*(i,k)-1}(i,k)
< 
\frac23 
<
y_{\ell^*(j,k)}(j,k)~.
\end{align*}
% Therefore, there is no violation of the ultrametric inequality in this triangle and the algorithm will not modify any low-error edges in $\mathcal{A}_t^1$. 

Accordingly, we define $B_{i,j,t}=B_{i,k,t}=B_{j,k,t}=0$ in this type, and Lemma~\ref{lem:M-bound-by-B} trivially holds for this type. 

\paragraph{Two Deterministic Edges (Type 2 \& 3).}
W.l.o.g, suppose $(i,j),(i,k)$ are the two deterministic edges. Then edge $(j,k)$ is high-error, and thus $M_{j,k,t}=0$. Next, we shall divide this case into two types: respectively, when $\ell^*(y,i,j)=\ell^*(y,i,k)$ and when $\ell^*(y,i,j)\neq \ell^*(y,i,k)$. Before the discussion of the two types, we shall introduce a useful lemma:
\begin{lemma}
\label{lem:y-bounded-by-c*}
In any recursive call that takes input $x$ and LP solution $y$, for any edge $(i,j)\in \binom{[n]}{2}$, $1-\Delta y_{\ell^*(i,j)}(i,j)\leq c^*(i,j)$. In particular, $y_{\ell^*(i,j)-1}(i,j)\leq c^*(i,j)$. 
\end{lemma}
\begin{proof}
For the initial LP solution $y^*$ and any edge $(i,j)\in \binom{[n]}{2}$, we have 
\begin{align*}
    c^*(i,j) = 1-\Delta y^*_{\ell(i,j)}(i,j) \geq 1-\Delta y^*_{\ell^*(i,j)}(i,j)~.
\end{align*}
Finally, because of Lemma~\ref{lem:delta-y-inc}, this lemma holds for any recursive call.
\end{proof}
Next, we discuss the two types. 
\begin{itemize}
\item \textbf{When $\ell^*(i,j)=\ell^*(i,k)$ (type 2).} In this case, $M_{i,j,t}=1$ only when the pivot is $k$ and the randomly sampled edge weight $x'(j,k)>w_{\ell^*(i,j)}$. When $k$ is the pivot, according to the CCDF, the probability that $x'({j,k})>w_{\ell^*(i,j)}$ is upper bounded by
\begin{align*}
    y_{\ell^*(i,j)-1}(j,k) 
    &
    \leq 
    y_{\ell^*(i,j)-1}(i,j) + y_{\ell^*(i,j)-1}(i,k)
    \\
    &
    =
    y_{\ell^*(i,j)-1}(i,j) + y_{\ell^*(i,k)-1}(i,k)
    \\
    &
    % \leq 
    % c(i,j) + c(i,k)
    \leq 
    c^*(i,j) + c^*(i,k)
\end{align*}
Because each vertex is chosen as the pivot with equal probability $\frac{1}{3}$ conditioned on $\mathcal{A}_t^2$, $\expect[M_{i,j,t}|\mathcal{A}_t^2]\leq \frac{1}{3}(c^*(i,j)+c^*(i,k))$. Since $(i,j)$ and $(i,k)$ are symmetric in this triangle, we can similarly show $\expect[M_{i,k,t}|\mathcal{A}_t^2]\leq \frac{1}{3}(c^*(i,j)+c^*(i,k))$. In total, we have
\begin{align*}
    \sum_{(u,v)\in t} \expect[M_{u,v,t}|\mathcal{A}_t^2]
    \leq 
    \frac{2}{3}(c^*(i,j)+c^*(i,k))
    ~.
\end{align*}
Accordingly, for edge $(u,v)$ equals $(i,j)$ or $(i,k)$, we define $B_{u,v,t}=1$ when it is the backward edge in the triangle. However, for edge $(j,k)$, because $c^*(j,k)$ is independent to the above bound of $M_{u,v,t}$, even when it is the backward edge, we still define $B_{j,k,t}=0$. Because each vertex is chosen as the pivot with each probability $\frac13$ conditioned on $\mathcal{A}_t^2$, we have $\expect[B_{i,j,t}|\mathcal{A}_t^2]=\expect[B_{i,k,t}|\mathcal{A}_t^2]=\frac{1}{3}$. Therefore, we derive the lemma for type 2.

\item \textbf{When $\ell^*(i,j)\neq \ell^*(i,k)$ (type 3).} W.l.o.g. suppose $(i,j)$ has higher deterministic weight, i.e. $\ell^*(i,j)<\ell^*(i,k)$. In this case, $M_{i,j,t}=1$ only when the pivot is $k$ and the randomly sampled edge weight $x'({j,k})\neq w_{\ell^*(i,j)}$. According to the CCDF, the probability that $x'({j,k})\neq w_{\ell^*(i,j)}$ is upper bounded by
\begin{align*}
    1 - \Delta y_{\ell^*(i,j)}(j,k)
    &
    = 
    1-y_{\ell^*(i,j)}(j,k)+y_{\ell^*(i,j)-1}(j,k)
    \\
    &
    \leq 
    1 - (y_{\ell^*(i,j)}(i,j) - y_{\ell^*(i,j)}(i,k)) + y_{\ell^*(i,j)-1}(i,j) + y_{\ell^*(i,j)-1}(i,k)
    \\
    &
    \leq 
    1 - y_{\ell^*(i,j)}(i,j) + y_{\ell^*(i,k)-1}(i,k) + y_{\ell^*(i,j)-1}(i,j) + y_{\ell^*(i,k)-1}(i,k)
    % \\
    % &
    % \leq 
    % c(i,j) + 2c(i,k)
    \\
    &
    \leq 
    c^*(i,j)+c^*(i,k)+c^*(j,k) 
    \tag{$c^*(j,k)\ge \frac13 > y_{\ell^*(i,k)-1}(i,k)$}
\end{align*}
Because each vertex is chosen as the pivot with equal probability $\frac{1}{3}$ conditioned on $\mathcal{A}_t^3$, $\expect[M_{i,j,t}|\mathcal{A}_t^3]\leq \frac{1}{3}(c^*(i,j)+c^*(i,k)+c^*(j,k))$. Observe that the pivot is $j$ and the random sampled edge weight $x'(j,k)\neq w_{\ell^*(i,j)}$ is a necessary condition for $M_{i,k,t}=1$. Similar by the above argument, we have $\expect[M_{i,k,t}|\mathcal{A}_t^3]\leq \frac{1}{3}(c^*(i,j)+c^*(i,k)+c^*(j,k))$. In total, we have
\begin{align*}
    \sum_{(u,v)\in t} \expect[M_{u,v,t}|\mathcal{A}_t^3]
    \leq 
    \frac{2}{3}(c^*(i,j)+c^*(i,k)+c^*(j,k))
    ~.
\end{align*}
Accordingly, for each edge $(u,v)\in t$, we define $B_{u,v,t}=1$ when it is the backward edge in the triangle. Because each vertex is chosen as the pivot with equal probability $\frac{1}{3}$ conditioned on $\mathcal{A}_t^3$, for each edge $(u,v)\in t$, $\expect[B_{u,v,t}|\mathcal{A}_t^3]=\frac{1}{3}$. Therefore, we derive the lemma for type 3.

\end{itemize}

\paragraph{One Deterministic Edge (Type 4).}
W.l.o.g., suppose $\Delta y_{\ell^*(j,k)}>\frac23$. Because $(i,j), (i,k)$ are high-error edges, $M_{i,j,t}=M_{i,k,t}=0$. Further, $M_{j,k,t}=1$ only when the pivot in the recursive call is $i$. Because each vertex is chosen as the pivot with equal probability $\frac{1}{3}$ conditioned on $\mathcal{A}_t^4$, $\expect[M_{i,j,t}|A^4_t] \leq \frac{1}{3}$. Therefore, $$\sum_{(u,v)\in t} \expect[M_{u,v,t}|\mathcal{A}_t^4]\leq \frac{1}{3}~.$$

Accordingly, for each $(u,v)\in t$, we define $B_{u,v,t}=1$ when it is the backward edge in the triangle. Since edges $(i,j)$ and $(i,k)$ are random and thus high-error, 
\begin{align*}
    \sum_{(u,v)\in t} c^*(u,v) \cdot \expect[B_{u,v,t}|\mathcal{A}_t^4] = \frac{1}{3}(c^*(i,j)+c^*(i,k)+c^*(j,k)) \geq \frac{2}{9}~. 
\end{align*}
Therefore, $\sum_{(u,v)\in t} \expect[M_{u,v,t}|\mathcal{A}_t^4] \leq 1.5 \sum_{(u,v)\in t} c^*(u,v) \cdot \expect[B_{u,v,t}|\mathcal{A}_t^4]$. 

Because each vertex is chosen as the pivot with equal probability $\frac{1}{3}$ conditioned on $\mathcal{A}_t$, if both $(i,j)$ and $(i,k)$ are $\lowerr$, $\sum_{(u,v)\in t} \expect[M_{u,v,t}|\mathcal{A}_t]$ can be upper bounded by $\frac{2}{3}$ times of Eqn.~\eqref{eqn:type-3-error}, and otherwise, it can be upper bounded by $\frac{1}{3}$ times of Eqn.~\eqref{eqn:type-3-error}. With the above lower bounds of the charges we defined, we can derive Lemma~\ref{lem:improved-M-bound-by-B} for this type. 
% On the other hand, if $(i,k)$ is $\higherr$, $c^*(i,j) \cdot \expect[B_{i,j,t}|\mathcal{A}_t]\geq \frac{1}{3}(1 - \Delta y_{\ell^*(i,j)}(i,j))$ and $c^*(i,k) \cdot \expect[B_{i,k,t}|\mathcal{A}_t]\geq \frac{1}{3}y_{\ell^*(i,k)-1}(i,k)$. Therefore, 

Conditioned on being backward in this type, $i,j$ (or, $i,k$) will appear in different clusters with probability at least $1-\alpha$, which can be lower bounded by (resp., for $B_{i,k,t}$)
\begin{align*}
    \begin{cases}
        \frac{1-\alpha}{2} B_{i,j,t} & \text{$(i,j)$ is $\lowerr$}\\
        \alpha B_{i,j,t} & \text{$(i,j)$ is $\highdet$}\\
        (1-\alpha)B_{i,j,t}  & \text{$(i,j)$ is $\highrand$}
    \end{cases}
\end{align*}
Because of $\alpha\geq \frac{1}{2}$, we derive Lemma~\ref{lem:improved-bound-of-B} for edges $(i,j)$ and $(i,k)$. On the other hand, because the deterministic weight of $(i,j)$ and $(i,k)$ are different, conditioned on being backward, $j,k$ will appear in different clusters with probability $1$, which equals $\frac{1}{2}B_{j,k,t}$ and lower bounded by $(1-\alpha)B_{j,k,t}$. Since random edges can only be $\highrand$, we derive Lemma~\ref{lem:improved-bound-of-B} for edge $(j,k)$. 
% , $\expect[M_{i,j,t}|\mathcal{A}_t^3]\leq \frac{1}{3}(c^*(i,j)+c^*(i,k)+c^*(j,k))$. Observe that the pivot is $j$ and the randomly sampled edge weight $x'(j,k)\neq w_{\ell^*(i,j)}$ is a necessary condition for $M_{i,k,t}=1$. Similar by the above argument, we have $\expect[M_{i,k,t}|\mathcal{A}_t^3]\leq \frac{1}{3}(c^*(i,j)+c^*(i,k)+c^*(j,k))$. In total, we have
% \begin{align*}
%     \sum_{(u,v)\in t} \expect[M_{u,v,t}|\mathcal{A}_t^3]
%     \leq 
%     \frac{2}{3}(c^*(i,j)+c^*(i,k)+c^*(j,k))
%     ~.
% \end{align*}
% Accordingly, for each edge $(u,v)\in t$, we define $B_{u,v,t}=1$ when it is the backward edge in the triangle. Because each vertex is chosen as the pivot with equal probability $\frac{1}{3}$ conditioned on $\mathcal{A}_t^3$, for each edge $(u,v)\in t$, $\expect[B_{u,v,t}|\mathcal{A}_t^3]=\frac{1}{3}$. Therefore, we derive the lemma for type 3.


\paragraph{No Deterministic Edge (Type 5).}
Because none of the edges are deterministic, none of the edges are low-error. Therefore, $M_{i,j,t}=M_{i,k,t}=M_{j,k,t}=0$. Accordingly, we define $B_{i,j,t}=B_{i,k,t}=B_{j,k,t}=0$ in this type, and Lemma~\ref{lem:M-bound-by-B} trivially holds for this type. 

\begin{algorithm}[H]
    \caption{$\umvd\text{-}\textsc{Pivot}(V, x, u)$}
    \label{alg:k-pivot}
    \DontPrintSemicolon
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    % \SetKwInOut{Parameter}{Parameter}
        
    % \Input{ $V\subseteq [n], ~u\in [L], ~x\in \mathbb{R}_{\geq 0}^{\binom{V}{2}}$} %,~ d\in \mathbb{R}_{\geq 0}^{[L]}, ~y^*\in \mathbb{R}_{\geq 0}^{\binom{V}{2}\times [L]}$}
    
    % \Output{ $x'\in \mathbb{R}_{\geq 0}^{\binom{V}{2}}$}
    
    % \Parameter{$\alpha\in [\frac{1}{2},1]$}
    
    \If{$|V|\leq 2$ \bf{or} $u=L$}{
    
        \Return{$x$}
    }
    
    $i\gets$ random vertex in $V$ 
    
    $y\gets y^*$

    \For{$i,j\in \binom{V}{2}$}{
        \For{$\ell\in [u-1]$}{
            $y_{\ell}(i,j)\gets 0$
        }
    }
    
    \For{$j\in V\setminus \{i\}$}{

        $\ell^*\gets \arg\max_{\ell\in [L]} ~\Delta y_\ell(i,j)$ \tcp*{break tie arbitrarily}
    
        \eIf{$(i,j)\in E$}{
            \eIf{$\Delta y_{\ell^*}({i,j}) > 1-\alpha$}{
                $x'(i,j)\gets d_{\ell^*}$ \tcp*{deterministic edges}
            }{
                $x'(i,j)\gets$ sampled according to Eqn.~\eqref{eqn:k-distance-ccdf} \tcp*{random edges}
            }
        }
        {
            \eIf{$\Delta y_{\ell^*}({i,j}) > 1-\beta\cdot \alpha$}{
                $x'(i,j)\gets d_{\ell^*}$ \tcp*{deterministic $\varnothing$ edges}
            }{
                $x'(i,j)\gets$ sampled according to Eqn.~\eqref{eqn:k-empty-distance-ccdf} \tcp*{random $\varnothing$ edges}
            }
        }
    }
    
    \For{$(j,k)\in \binom{V\setminus \{i\}}{2}$}{
        \eIf{$x'({i,j})=x'({i,k})$}{
            $x'({j,k})\gets \min\{x({j,k}),x'({i,j})\}$
        }{
            $x'({j,k})\gets \max\{x'({i,j}),x'({i,k})\}$
        }
    }
    
    \For{$\ell\in \{u,u+1,\cdots,L\}$}{
        $V_\ell\gets \{j\in V: x'({i,j})=d_{\ell}\}$ \label{line:k-partition-non-pivots}
    
        $x'\big|_{\binom{V_\ell}{2}}\gets \umvd\text{-}\textsc{Pivot}\Big(V_\ell, x'\big|_{\binom{V_\ell}{2}}, \ell\Big)$ %, d, y^*\big|_{\binom{V_{\ell}}{2}\times [L]}\Big)$
    }
    
    \Return{$x'$}
\end{algorithm}

\begin{align}
    \label{eqn:k-distance-ccdf}
    \forall i\in [L],\quad \Pr[x'(i,j)\geq d_{\ell}] = \frac{1}{1-\beta \cdot \alpha}\cdot \max\big\{0,~ y_{\ell}(i,j)-\beta \cdot \alpha\big\}~.
\end{align}
\begin{align}
    \label{eqn:k-empty-distance-ccdf}
    \forall i\in [L],\quad \Pr[x'(i,j)\geq d_{\ell}] = y_\ell(i,j)~.
\end{align}
